Dividing and Conquering a BlackBox to a Mixture of Interpretable Models: Route, Interpret, Repeat

ML model design either starts with an interpretable model or a Blackbox and explains it post hoc. Blackbox models are flexible but difficult to explain, while interpretable models are inherently explainable. Yet, interpretable models require extensive ML knowledge and tend to be less flexible and underperforming than their Blackbox variants. This paper aims to blur the distinction between a post hoc explanation of a Blackbox and constructing interpretable models. Beginning with a Blackbox, we iteratively carve out a mixture of interpretable experts (MoIE) and a residual network. Each interpretable model specializes in a subset of samples and explains them using First Order Logic (FOL), providing basic reasoning on concepts from the Blackbox. We route the remaining samples through a flexible residual. We repeat the method on the residual network until all the interpretable models explain the desired proportion of data. Our extensive experiments show that our route, interpret, and repeat approach (1) identifies a diverse set of instance-specific concepts with high concept completeness via MoIE without compromising in performance, (2) identifies the relatively ``harder'' samples to explain via residuals, (3) outperforms the interpretable by-design models by significant margins during test-time interventions, and (4) fixes the shortcut learned by the original Blackbox. The code for MoIE is publicly available at: \url{https://github.com/batmanlab/ICML-2023-Route-interpret-repeat}

==> Sections/abstract_v1.tex <==
The current approach to ML model design is either to choose a flexible Blackbox model and explain it post hoc or to start with an interpretable model. 
Blackbox models are flexible but difficult to explain, whereas interpretable models are designed to be explainable. 
However, developing interpretable models necessitates extensive ML knowledge, and the resulting models tend to be less flexible, offering potentially subpar performance compared to their Blackbox equivalents. 
This paper aims to blur the distinction between a post hoc explanation of a BlackBox and constructing interpretable models. 
We propose beginning with a flexible BlackBox model and gradually \emph{carving out} a mixture of interpretable models and a \emph{residual network}. 
Our design identifies a subset of samples and \emph{routes} them through the interpretable models. The remaining samples are routed through a flexible residual network. 
We adopt First Order Logic (FOL) as the interpretable model's backbone, which provides basic reasoning on concepts retrieved from the BlackBox model. 
On the residual network, we repeat the method until the proportion of data explained by the residual network falls below a desired threshold. 
Our approach offers several advantages. First, the mixture of interpretable and flexible residual networks results in almost no compromise in performance. Second, the route, interpret, and repeat approach yields a highly flexible interpretable model. 
Our extensive experiment demonstrates the performance of the model on various datasets. We show that by editing the FOL model, we can fix the shortcut learned by the original BlackBox model. 
Finally, our method provides a framework for a hybrid symbolic-connectionist network that is simple to train and adaptable to many applications.

==> Sections/baseline_v1.tex <==
We compare our methods to two baselines -- 1) interpretable by design 2) posthoc concept bottlenecks (PCBMs). For interpretable by design, we employ the end to end concept embedding models (CEMs)~\cite{zarlenga2022concept} and sequential concept bottleneck models (CBMs)~\cite{koh2020concept}, consisting of two parts: 1) a concept extractor $\phi: \mathcal{X} \rightarrow \mathcal{C}$, predicting concepts from images; and 2) a classifier $g: \mathcal{C} \rightarrow \mathcal{Y}$, predicting labels from the concepts. Convolution-based $\phi$ includes all layers till the last convolution block. VIT-based $\phi$ consists of the transformer encoder block (excluding the classification head). For PCBMs, we employ the similar strategy described in~\cite{yuksekgonul2022post} to classify using the extracted the concepts from image embeddings of a trained blackbox. Furthermore, we use the identical $g$ of MOIE (as in Appendix \ref{app:g}) replacing the label predictors of CBM and PCBM to compare our FOL explanations with the baselines. Henceforth, we refer them as CBM + ELL and PCBM + ELL. As~\cite{barbiero2022entropy} trains the concept and label predictors sequentially, we also perform the same for the CBM + ELL and PCBM + ELL baselines. For HAM10000 dataset, we extract the concepts from Derm7pt dataset using the pretrained embeddings of the blackbox as per~\cite{yuksekgonul2022post}. Thus, we can not use interpretable by design baselines for HAM10000 and SIIM-ISIC due to the unavailability of concept annotations in the dataset.

==> Sections/intro_v1.tex <==
 
Model explainability is essential in high-stakes applications of AI, such as healthcare. While BlackBox models (\eg Deep Learning) offer flexibility and modular design, post hoc explanation is prone to confirmation bias~\cite{wan2022explainability}, lack of fidelity to the original model~\cite{adebayo2018sanity}, and insufficient mechanistic explanation of the decision-making process~\cite{rudin2019stop}. Interpretable-by-design models do not suffer from those issues but tend to be less flexible than Blackbox models and demand substantial expertise to design and fine-tune. Using post hoc explanation or adopting an interpretable model is a mutually exclusive decision to be made at the initial phase of AI model design. This paper aims to blur the line on that dichotomous model design. 

The literature on post hoc explainable AI is extensive. The methods such as model attribution (\eg Saliency Map~\cite{simonyan2013deep, selvaraju2017grad}), counterfactual approach ~\cite{abid2021meaningfully, singla2019explanation}, and distillation methods~\cite{alharbi2021learning, cheng2020explaining} are examples of post hoc explainability approaches. Those methods either identify important features of input that contribute the most to the network's output~\cite{shrikumar2016not}, generate perturbation to the input that flips the network's output~\cite{samek2016evaluating}, \cite{montavon2018methods}, or estimate simpler functions that locally approximate the network output. The advantage of the post hoc explainability methods is that they do not compromise the flexibility and performance of the BlackBox. However, the post hoc explainability method suffers from several undesirable significant drawbacks, such as a lack of fidelity and mechanistic explanation of the network output~\cite{rudin2019stop}. Without a mechanistic explanation, recourse to a model's undesirable behavior is unclear. Interpretable models are alternative designs to the BlackBox model that do not suffer from many of those drawbacks. 

Interpretable models also have a long history in statistics and machine learning~\cite{letham2015interpretable, breiman1984classification}. Several families of interpretable models exist, such as the rule-based approach and generalized additive models~\cite{hastie1987generalized}. Many methods focus on tabular or categorical data and less on high-dimensional structured data such as images. Interpretable models for structured data rely mostly on projecting to a lower dimensional \emph{concept} or \emph{symbolic} space that is understandable for humans~\cite{koh2020concept}. Aside from a few exceptions ~\cite{ciravegna2021logic, barbiero2022entropy}, the current State-Of-The-Art (SOTA) design does not model the interaction between concepts and symbols, hence offering limited reasoning capabilities and less robustness. Furthermore, current designs are not as flexible as the Blackbox model, which may compromise the performance of such models. 


We aim to achieve the best of both worlds: the flexibility of the BlackBox and the mechanistic explainability of the interpretable models. The general idea is that a single interpretable model may not be sufficiently powerful to explain all samples, and several interpretable models might be hidden inside the Blackbox model. We construct a hybrid neuro-symbolic model by progressively \emph{carving out} a mixture of interpretable model and a \emph{residual network}. Our design identifies a subset of samples and \emph{routes} them through the interpretable models. The remaining samples are routed through a flexible residual network. We adopt First Order Logic (FOL) as the interpretable model's backbone, which provides basic reasoning on concepts retrieved from the BlackBox model. 
FOL is a logical function
that accepts predicates (concept presence/absent) as input and returns a True/False output being a
logical expression of the predicates. The logical expression, which is a set of AND, OR, Negative,
and parenthesis, can be written in the so-called Disjunctive Normal Form (DNF). DNF is a FOL logical formula composed of a disjunction (OR) of conjunctions (AND), known as the ``sum of products''.
On the residual network, we repeat the method until the proportion of data explained by the residual network falls below a desired threshold. The experimental results across various computer vision and medical imaging datasets reveal that our method accounts for the diversity of the explanation space and has minimal impact on the Blackbox's performance. Additionally, we apply our method's explanations to detect shortcuts in computer vision and successfully eliminate the bias from the Blackbox's representation.

\paragraph{Contributions}
% \begin{figure}[t]
% \centering
% \includegraphics[width=1\textwidth]{figures/Final/Local_explanation_motivation.pdf}
% \caption{The motivation of our work. All the plots correspond to detect a skin lesion as ``Malignant". In the left, (a) plot of the weights for each concepts by the fully interpretable model; (b) explanations by the interpretable model containing the concept \textit{sex} as it has the height weight, making the explanation too generic; (c) plot of the weights for each concepts by the expert4 using our method; (d) explanations by the expert4 using our method; (e) plot of the weights for each concepts by the expert5 using our method; (f) explanations by the expert5 using our method. From (c)-(f), we can see the expert model focuses on specific concept for specific samples.}
% \label{fig:motivation} 
% \end{figure}

==> Sections/method_v1.tex <==

\textbf{Notation and learning the concepts:} 
Assume $f^0: \mathcal{X} \rightarrow \mathcal{Y}$ is a pre-trained Blackbox predicting the output from the input image. Also, $\displaystyle f^0(.) =  h^0 \circ \Phi(.) $. Here, $ \Phi: \mathcal{X} \rightarrow R^l $ is the image embeddings and $ h^0: R^l \rightarrow \mathcal{Y}$ is the classifier, classifying the output $\mathcal{Y}$ using the embeddings, $\Phi$. Our approach is applicable for both datasets with and without human-interpretable concept annotations. For datasets with the concept annotation $\mathcal{C} \in \mathbb{R}^{N_c}$ ($N_c$ being the number of concepts per image $\mathcal{X}$), we learn $t: R^l \rightarrow\mathcal{C}$ to classify the concepts using the embeddings. Per this definition, $t$ outputs a scalar value $c$ representing a single concept for each input image. 
%We adopt the concept learning strategy in PosthocCBM (PCBM)~\cite{yuksekgonul2022post} for datasets without concept annotation. 
%Specifically, we leverage a set of image embeddings with the concept being present and absent. Next, we learn a linear SVM to construct the concept activation matrix~\cite{kim2017interpretability} as $\boldsymbol{Q} \in\mathbb{R}^{N_c \times l}$. 
Finally we estimate the concept value as $c = \frac{<\Phi(x), q^i>}{||q_i||_2^2}$ $ \in \mathbb{R}$ utilizing each row $\boldsymbol{q^i}$ of $\boldsymbol{Q}$. Thus, the complete tuple of $j^{th}$ sample is $\{x_j, y_j, c_j\}$, denoting the image, label, and learned concept vector, respectively.

\textbf{Method Overview:} 
Figure \ref{fig:Schematic} summarizes our approach. We iteratively carve out an interpretable model from the given Blackbox. Each iteration yields an interpretable model (the downward grey paths in Figure \ref{fig:Schematic}) and a residual (the straightforward black paths in Figure \ref{fig:Schematic}).
We start with the initial Blackbox $f^0$.
At iteration $k$, we distill the Blackbox from the previous iteration $f^{k-1}$ into a neuro-symbolic interpretable model, $\displaystyle g^{k}: \mathcal{C} \rightarrow \mathcal{Y}$. Our $g$ is flexible enough to be any interpretable models \eg logistic classifier~\cite{yuksekgonul2022post, koh2020concept, barbiero2022entropy}. The \emph{residual} $r^k =f^{k-1} - g^k$ emphasizes the portion of $f^{k-1}$ that $g^k$cannot explain. We then approximate $r^k$ with $f^{k} = h^k(\Phi(.))$. $f^k$ will be the Blackbox for the subsequent iterations and be explained by the respective interpretable model. 
% Due to computational reasons, we only finetune $h^{k}$ to optimize for $r^k$. 
A learnable gating mechanism, denoted by $\pi^k : \mathcal{C} \rightarrow \{0,1\}$ (shown as the \emph{selector} in figure \ref{fig:Schematic}) routes an input sample towards either $g^k$ or $r^k$.
% In order to learn $\pi^k$, we use simple backpropagation while learning $g^k$. A
The thickness of the lines in Figure \ref{fig:Schematic} represents the samples covered by the interpretable models (grey line) and the residuals (black line). 
% Our method is designed such that it leaves a little number of samples for the last residual blackbox.
With every iteration, the cumulative coverage of the interpretable models increases, but the residual decreases. We name our method \emph{route, interpret} and \emph{repeat}.

\subsection{Neuro-Symbolic Knowledge Distillation}
Knowledge distillation in our method involves 3 parts: (1) a series of trainable selectors ,\emph{routing} each sample through the interpretable models and the residual networks, (2) A sequence of learnable neuro-symbolic interpretable models, each providing FOL explanations to \emph {interpret} the Blackbox, and (3) \emph{repeating} with Residuals for the samples that cannot be explained with their interpretable counterparts. 
We detail each component below.

\begin{figure}[h]
% \vskip 0.2in
\centering
\includegraphics[width=\columnwidth]{figures/main/schematic.pdf}
\vskip -3pt
\caption{Schematic view of \emph{route, interpret} and \emph{repeat}. At iteration $k$, the selector \emph{routes} each sample either towards the interpretable model $g^k$ (to \emph{interpret}) with probability $\pi^k(.)$ or the residual $r^k = f^{k-1} - g^k$ with probability $1-\pi^k(.)$ (to \emph{repeat} in the further iterations). $f^{k-1}$ is the Blackbox of the $(k-1)^{th}$ iteration. $g^k$ generates FOL-based explanations for the samples it covers. Otherwise, the selector routes through the next step until it either goes through a subsequent interpretable model or reaches the last residual. Also, components in black and grey indicate the fixed and trainable modules in our model respectively. }
\label{fig:Schematic} 
\vskip -0.1in
\end{figure}

\subsubsection{The selector function}
As the first step of our method, the selector $\pi^k$ \emph{routes} the $j^{th}$ sample through the interpretable model $g^k$ or residual $r^k$ with probability $\displaystyle \pi^k(\boldsymbol{c_j})$ and $\displaystyle 1 - \pi^k(\boldsymbol{c_j})$ respectively, where $k$ $\in [0,K]$, with $K$ being the number of iterations.
We define the empirical coverage of the $\displaystyle k^{th}$ iteration as $\vspace{-0.08pt} \zeta(\pi^k) = \frac{1}{m}\sum_{j = 1} ^ m \pi^k(\boldsymbol{c_j}) \vspace{-0.081pt}$, the empirical mean of the samples selected by the selector for the associated interpretable model $\displaystyle g^k$, with $\displaystyle m$ being the total number of samples in the training set. Thus, the entire selective risk is:

\vskip -7.5pt
\begin{equation}
\label{equ: emp_risk}
\mathcal{R}^k(\displaystyle \pi^k, \displaystyle g^k) = \frac{\frac{1}{m}\sum_{j=1}^m\mathcal{L}_{(g^k, \pi^k)}^k\big(\boldsymbol{x_j}, \boldsymbol{c_j}\big)}{\zeta(\pi^k)} ,
\end{equation}
\vskip 2pt

where $\mathcal{L}_{(g^k, \pi^k)}^k$ is the optimization loss used to learn $\displaystyle g^k$ and $\displaystyle \pi^k$ together, discussed in section \ref{ns-optimization}. For a given coverage of $\displaystyle \tau^k \in (0, 1]$, we solve the following optimization problem:

\vskip -7.5pt
\begin{align}
\label{equ: optimization_g}
\theta_{s^k}^*, \theta_{g^k}^* = & \operatorname*{arg\,min}_{\theta_{s^k}, \theta_{g^k}} \mathcal{R}^k\Big(\pi^k(.; \theta_{s^k}), \displaystyle g^k(.; \theta_{g^k}) \Big) \nonumber \\ 
&\text{s.t.} ~~~ \zeta\big(\pi^k(.; \theta_{s^k})\big) \geq \tau^k,
\end{align}
\vskip 2pt

where $\theta_{s^k}^*, \theta_{g^k}^*$ are the optimal parameters at iteration $k$ for the selector $\pi^k$ and the interpretable model $g^k$ respectively. In this work, $\pi$s' of different iterations are neural networks with sigmoid activation. At inference time, the selector routes the $j^{th}$ sample with concept vector $\boldsymbol{c_j}$ to $\displaystyle g^k$ if and only if $\pi^k(\boldsymbol{c}_j)\geq 0.5$ for $k \in [0,K]$.

\subsubsection{Neuro-Symbolic interpretable models}
\label{ns-optimization}
In this stage, we design interpretable model $\displaystyle g^k$ of $k^{th}$ iteration  to \emph{interpret} the Blackbox $\displaystyle f^{k - 1}$ from the previous $(k-1)^{th}$ iteration by optimizing the following loss function:
\begin{equation}
\label{equ: g_k}
\resizebox{0.47\textwidth}{!}{$
\mathcal{L}_{(g^k, \pi^k)}^k\big(\boldsymbol{x_j}, \boldsymbol{c_j}\big) = \underbrace{\mystrut{2.6ex}\ell\Big(f^{k - 1}(\boldsymbol{x_j}), g^k(\boldsymbol{c_j})\Big)\pi^k(c_j) }_{\substack{\text{trainable component} \\ \text{for current iteration $k$}}}\underbrace{\prod_{i=1} ^{k - 1}\big(1 - \pi^i(\boldsymbol{c_j})\big)}_{\substack{\text{fixed component trained} \\ \text{in the previous iterations}}},
$}
\end{equation}

where the term $\pi^k(\boldsymbol{c_j})\prod_{i=1} ^{k - 1}\big(1 - \pi^i(\boldsymbol{c_j}) \big)$ denotes the probability of $j^{th}$ sample being routed through the interpretable model $g^k$. It is the probability of the sample going through the residuals for all the previous iterations from $0$ through $k-1$ (\ie $\prod_{i=1} ^{k - 1}\big(1 - \pi^i(\boldsymbol{c_j}) \big)$\big) times the probability of going through the interpretable model at iteration $k$ \big(\ie $\pi^k(\boldsymbol{c_j})$\big). 
Refer to Figure~\ref{fig:Schematic} for an illustration. We learn $\pi^1, \dots \pi^{k - 1}$ in the prior iterations and are not trainable at iteration $k$. As each interpretable model $g^k$ specializes in explaining a specific subset of samples (denoted by coverage $\tau$), we refer to it as an \emph{expert}. We use SelectiveNet's ~\cite{geifman2019selectivenet}  optimization method to optimize equation \ref{equ: optimization_g} since selectors need a rejection mechanism to route samples through residuals. Appendix \ref{app:loss} details the optimization procedure in equation \ref{equ: g_k}. We refer to the interpretable experts of all the iterations as a ``Mixture of Interpretable Experts'' (MoIE) cumulatively after training. Furthermore, we utilize Entropy-based linear layer neural network (ELL)~\cite{barbiero2022entropy} as the interpretable symbolic model $g$ to construct First Order Logic (FOL) explanations of a given prediction.

\subsubsection{The Residuals}
The last step is to \emph{repeat} with the residual $r^k$, as $\displaystyle r^k(\boldsymbol{x_j},\boldsymbol{c_j}) = f^{k - 1}(\boldsymbol{x_j}) - g^k(\boldsymbol{c_j})$.
We train $f^k = h^k\big(\Phi(.)\big)$ to approximate the residual $r^k$, creating a new Blackbox $f^k$ for the next iteration $(k+1$). This step is necessary to specialize $\displaystyle f^k$ over samples not covered by $g^k$. Optimizing the following loss function yields $\displaystyle f^k$ for the $\displaystyle k^{th}$ iteration:
\begin{equation}
\label{equ: residual}
\mathcal{L}_f^k(\boldsymbol{x_j}, \boldsymbol{c_j}) = \underbrace{\mystrut{2.6ex}\ell\big(r^k(\boldsymbol{x_j}, \boldsymbol{c_j}), f^k(\boldsymbol{x_j})\big)}_{\substack{\text{trainable component} \\ \text{for iteration $k$}}} \underbrace{\mystrut{2.6ex}\prod_{i=1} ^{k}\big(1 - \pi^i(\boldsymbol{c_j})\big)}_{\substack{\text{non-trainable component} \\ \text{for iteration $k$}}} 
\end{equation}

% \underbrace{\mystrut{2.6ex}\ell\big(f^{k - 1}(\boldsymbol{x_j}), g^k(\boldsymbol{c_j})\big)\pi^k(c_j) }_{\substack{\text{trainable component} \\ \text{from current iteration}}}
Notice that we fix the embedding $\displaystyle \Phi(.)$ for all the iterations. Due to computational overhead, we only finetune the last few layers of the Blackbox ($h^k$) to train $f^k$.
At the final iteration $K$, our method produces a MoIE and a Residual, explaining the interpretable and uninterpretable components of the initial Blackbox $f^0$, respectively. Appendix \ref{app:algo} describes the training procedure of our model, the extraction of FOL and the architecture of our model at inference.


\textbf{Selecting number of iterations $K$:} We follow two principles to select the number of iterations $K$ as a stopping criterion: 1) Each expert should have enough data to be trained reliably (
coverage $\zeta^k$). If an expert covers insufficient samples, we stop the process. 2) If the final residual ($r^K$) underperforms a threshold, it is not reliable to distill from the Blackbox. We stop the procedure to ensure the overall accuracy is maintained.

==> Sections/related_work_v1.tex <==
% Post hoc methods
% Saliency cam grad cam
% attribution lime shap l2x

% interpretable models
% early GAM - tabular data
% CBM no composability
% E-LENS FOL

\textbf{Post hoc explanations:} \cite{simonyan2013deep, selvaraju2017grad, smilkov2017smoothgrad} discuss the post hoc explanation method using saliency maps to explain a convolution neural network, highlighting the pixels in the input images that contributed to the network's prediction. \cite{adebayo2018sanity, kindermans2019reliability}  demonstrates that the saliency maps highlight the correct regions in the image even though the backbone's representation was arbitrarily perturbed. Additionally, in LIME~\cite{ribeiro2016should}, given a superpixel, a surrogate linear function attempts to learn the prediction of the Blackbox surrounding that superpixel. SHAP \cite{SHAP} utilizes a game-theoretic strategy called SHAPLY values to estimate the Blackbox's prediction by considering all the permutations of adding and removing a specific feature to determine its importance in the final prediction. Regarding pixel intensities, the explanations do not correspond to the high-level, human-interpretable \emph{concepts}. In this paper, we provide the post hoc explanation of the Blackbox in terms of the interpretable concepts, rather than the pixel intensities.

% \textbf{Concept-based interpretable models}: 
% In this class, the researchers try to design inherently interpretable models to eliminate the  requirement for post hoc explanations. In the literature, we find interpretable models in Generalized Additive Models (GAM)~\cite{hastie1987generalized}, or on logic formulas, as in Decision Trees~\cite{breiman1984classification} or Bayesian Rule Lists (BRL)~\cite{letham2015interpretable}. 
% % GAMs overcome the linearity assumption of linear regression by learning target categories disjointly from each feature. 
% However, most of these methods work well in categorical datasets rather than continuous data such as images. Additionally,~\cite{chen2019looks} introduces a ``case-based reasoning'' technique, known as ``ProtoPNet''. Here, the authors first dissect an image in Prototypical parts and then classifies by combining evidence from the pre-defined prototypes. This method is highly sensitive to the choice of prototypes and the distance metric used to compare with the prototype. So instead of using any prototypes, our proposed method uses human understandable concepts to build the mixture of interpretable models.
\textbf{Concept-based interpretable models:}
Recently, CBM~\cite{koh2020concept}, based on the interpretable-by-design principle, leverages the weak annotations of visual attributes to predict the high-level human-comprehensible concepts~\cite{kim2017interpretability} from images and then the class labels from the discovered concepts. A concept decoder is used in the antehoc model~\cite{sarkar2021inducing} to simultaneously reconstruct the image from the concepts to ensure the the semantics of the input image from the concepts, specifically aiming for unsupervised concept discovery. Instead of learning scalar concepts in the bottleneck, CEM~\cite{zarlenga2022concept} uses high dimensional concept embeddings to allow extra supervised learning capacity. Later,PCBM ~\cite{yuksekgonul2022post} learns the concepts from the embeddings of a trained Blackbox and uses an interpretable classifier for classification. Also, they propose the Hybrid-Post-hoc-concept-based model (PCBM-h) to replicate the performance of the Blackbox. Yet, they do not explain how the final classifier composes those concepts for prediction. An inherently interpretable ELL~\cite{barbiero2022entropy} addresses this gap by introducing an entropy-based classifier for the downstream classification and providing explanations in terms of FOL using the concepts. However, all these methods 1) employ a single interpretable model to explain a Blackbox, failing to apprehend different forms of explanations for different samples and offering generic explanations for all samples of a class 2) did not quantify if the identified concepts is faithful to the Blackbox's prediction. We introduce MoIE to address this issue, utilizing Blackbox's flexibility to identify meaningful instance-specific concepts with high concept completeness to offer a local explanation using FOL. In addition, we learn the residuals in each iteration for the samples not covered by the associated interpretable model, whereas PCBM-h trains the residual for all samples.

\textbf{Shortcut learning:}
"Shortcuts'' are defined when a predictor relies on easy-to-learn spurious correlations between the inputs and the target~\cite{geirhos2020shortcut}. Learning shortcuts can broadly be categorized either in example difficulty estimation~\cite{lalor2018understanding, hooker2019compressed, agarwal2022estimating} or monitoring training dynamics~\cite{hu2020surprising, feng2021phases, rabanser2022selective}. Unlike these methods, MoIE discovers shortcut using the high level concepts in FOL explanation of the Blackbox's prediction of a sample, routed through an interpretable model and eliminate it using MDN \cite{lu2021metadata}.

==> Sections/related_work_v2.tex <==
% Post hoc methods
% Saliency cam grad cam
% attribution lime shap l2x

% interpretable models
% early GAM - tabular data
% CBM no composability
% E-LENS FOL

\textbf{Post hoc explanations:} 
Related work in Post-hoc explanation techniques include: 1) highlighting relevant pixels in the image~\cite{simonyan2013deep, selvaraju2017grad, smilkov2017smoothgrad, sundararajan2017axiomatic, binder2016layer}, 2) developing a surrogate linear function~\cite{ribeiro2016should, yoon2019rl} to imitate the Blackbox around a local neighborhood, and 3) using the game-theoretic SHAPLY values~\cite{SHAP} to determine feature importance in the Blacbox prediction. Though post hoc explanations retain the flexibility and performance of the Blackbox, they operate in pixel space, often not corresponding to humanly interpretable \emph{concepts}~\cite{kim2017interpretability}. This restricts the use of post-hoc methods in algorithmic recourse~\cite{bordt2022post}. In this paper, we offer a post hoc explanation of the Blackbox in terms of concepts to improve interpretability and facilitate test-time interventions on the concepts.

\textbf{Concept-based interpretable models:}
Concept-based interpretable models leverage the weak annotations of visual attributes to predict the concepts from images and then the class labels from the concepts, as in Concept Bottleneck models (CBMs)~\cite{koh2020concept}. A concept decoder is used in the antehoc model~\cite{sarkar2021inducing} to simultaneously reconstruct the image from the concepts to ensure the semantics of the input image from the concepts, specifically aiming for unsupervised concept discovery. Instead of learning scalar concepts in the bottleneck, end-to-end Concept Embedding models (CEMs)~\cite{zarlenga2022concept} uses high dimensional concept embeddings to allow extra supervised learning capacity and achieves SOTA performance in the interpretable-by-design class. An inherently interpretable ELL~\cite{barbiero2022entropy} introduces an entropy-based classifier for the downstream classification and provides explanations in terms of FOL using the concepts. Recently, Posthoc Concept Bottleneck models (PCBMs) ~\cite{yuksekgonul2022post} learn the concepts from a trained Blackbox  embeddings and uses an interpretable classifier for classification. Also, they fit a residual in their hybrid variant (PCBM-h) to mimic the performance of the Blackbox. However, all these methods employ a single interpretable model to explain a Blackbox. Thus, they offer generic explanations for all the samples of a class, lowering the performance, particularly for models that are inherently interpretable. Also PCBMs do not provide any reasoning through the identified concepts. Our MoIE overcomes these issues by 1) employing multiple experts to carve instance-specific concepts from the Blackbox while preserving its flexibility and performance, 2) providing fundamental reasoning on concepts by offering FOL explanations per sample, 3) fitting residuals in each iteration to progressively cover samples in an increasing order of ``hardness''.

\textbf{Shortcut learning:}
Often, a Blackbox leverages spurious correlations, having no semantic connection to the actual task. These spurious correlations are termed as ``shortcuts''.  that the model exploits for its decision without any connection to the actual task. Related work in explainability includes LIME~\cite{ribeiro2016should}, utilized to detect spurious background as a shortcut to classify an animal. Recently interpretable model~\cite{rosenzweig2021patch}, involving local image pathces, are used as a proxy to the Blackbox to identify shortcuts. However, both of them function in pixel space, notconcept space. Also, they do not eliminate the shortcut.  Our MoIE discovers shortcuts using the high level concepts in the FOL explanation of the Blackbox's prediction and eliminates them via Meta data normalization (MDN)~\cite{lu2021metadata}.

==> Sections/shortcut.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\textwidth]{figures/Final/shortcut.pdf}
\caption{Applying MoIE to eliminate shortcuts. (a) Performance of the biased Blackbox. 
(b) Performance of final MoIE, trained using the supervision of the robust Blackbox after removing the shortcuts using MDN. 
(c) Examples of samples and their explanations by the biased (top-row) and robust Blackboxes(bottom-row). 
(d) auroc and (e) accuracy metrics of the biased Blackbox (when the shortcuts are present) and the robust Blackbox (when the shortcuts are removed using MDN).
}
\label{fig:shortcut}
\end{figure}

To conduct this experiment, we create the Waterbirds dataset as in~\cite{sagawa2019dro} by spuriously correlating the images of birds from the Caltech-UCSD Birds-200-2011 dataset to the images of land and water background from the Places dataset. Specifically, we use forest and bamboo as the spurious land concepts for landbirds; ocean and lakes as the spurious water concepts for waterbirds. Thus, we have 112 visual concepts (108 concepts from CUB-200 and four new concepts for the background). We aim to identify each bird as a Waterbird or a Landbird. We use ResNet50 (\cite{he2016deep}) as the Blackbox $f^0$. The Blackbox quickly latches on the spurious background to classify the birds. As a result, the black box's accuracy varies for land-based subsets versus aquatic subsets of the bird species, as shown in figure \ref{fig:shortcut}a. The Waterbird on water is more accurate than on land ((96\%  vs. 67 \% in the orange bar in the figure \ref{fig:shortcut}a). We train $t$ to retrieve the concepts from the biased Blackbox. Next, we train our MoIE to explain the bird species using FOL. As per figure \ref{fig:shortcut}c (middle row), the FOL of a waterbird misclassified as a landbird captures the spurious concept \textit{forest}. Assuming the background concepts as metadata,  we aim to reduce the background bias from the representation of the Blackbox using metadata normalization (MDN) \cite{lu2021metadata}. Therefore, we leverage the MDN layers between two successive layers of the convolutional backbone to fine-tune the biased Blackbox. Next, we train $t$, using the embedding $\phi$ of the robust Blackbox. Figures \ref{fig:shortcut}d-e compare the auroc and accuracy scores of the spurious background concepts from the embedding $\phi$ of the biased and robust Blackboxes, respectively. The validation auroc (accuracy) of all the spurious concepts retrieved from the robust Blackbox fell well short of the predefined threshold 0.7 (70 \%) compared to the biased Blackbox. Finally, we re-train the MoIE distilling from the new robust Blackbox. Figure \ref{fig:shortcut}b illustrates that the accuracies of Waterbird on water vs. Waterbird on land become pretty similar (91\% -88 \%). The FOL from the robust Blackbox does not include any background concepts (Figure \ref{fig:shortcut}c, bottom row). Refer to the figure \ref{fig:spurious_flow} in Appendix \ref{app:shortcut} for the flow diagram of this experiment.
